Accelerating Java Ray Tracing Applications on Heterogeneous Hardware

Ray tracing has been typically known as a graphics rendering method capable of producing highly realistic imagery and visual effects generated by computers. More recently the performance improvements in Graphics Processing Units (GPUs) have enabled developers to exploit sufficient computing power to build a fair amount of ray tracing applications with the ability to run in real-time. Typically, real-time ray tracing is achieved by utilizing high performance kernels written in CUDA, OpenCL, and Vulkan which can be invoked by high-level languages via native bindings; a technique that fragments application code bases as well as limits portability. This paper presents a hardware-accelerated ray tracing rendering engine, fully written in Java, that can seamlessly harness the performance of underlying GPUs via the TornadoVM framework. Through this paper, we show the potential of Java and acceleration frameworks to process in real time a compute intensive application. Our results indicate that it is possible to enable real time ray tracing from Java by achieving up to 234, 152, 45 frames-per-second in 720p, 1080p, and 4K resolutions, respectively.

==> sections/abstract.tex <==
\begin{abstract}
Ray tracing has been typically known as a graphics rendering method capable of producing highly realistic imagery and visual effects generated by computers.
More recently the performance improvements in Graphics Processing Units (GPUs) have enabled developers to exploit sufficient computing power to build a fair amount of 
ray tracing applications with the ability to run in real-time.
Typically, real-time ray tracing is achieved by utilizing high performance kernels written in CUDA, OpenCL, and Vulkan which can be invoked by high-level languages via native bindings; a technique that fragments application code bases as well as limits portability.
    
This paper presents a hardware-accelerated ray tracing rendering engine, fully written in Java, that can seamlessly harness the performance of underlying GPUs via the TornadoVM framework.
Through this paper, we show the potential of Java and acceleration frameworks to process in real time a compute intensive application.
Our results indicate that it is possible to enable real time ray tracing from Java by achieving up to 234, 152, 45 frames-per-second in 720p, 1080p, and 4K resolutions, respectively.
\end{abstract}

==> sections/implementation.tex <==
\section{Implementation}

\jf{Candidate to move this section to Design Section}

% In this section, a deeper look into implementation decisions and architectural details are provided that encompass the development phase of the ray tracing application.

% \subsection{Data structures \& representations}

% As one of the objectives of the project was achieving real-time rendering performance, representing data values with the most efficient data structures was a key requirement throughout the implementation of the application. Some of the major decisions made are outlined as follows:

% \subsubsection{Floating-point precision}

% The wide use of non-integer values throughout the implementation of the rendering engine requires a decision to specify the type of floating point numbers utilized.

% While modern GPUs have support for both single and double precision floating point operations, latest families of graphics processing units exhibit magnitudes of performance differences in using the former over the latter: Nvidia's Geforce RTX 20 series show a 32x, while the newest Geforce RTX 30 series show a 64x faster single precision floating point operations per second measurement compared to double precision \cite{wiki:GeForce_20_series} \cite{wiki:GeForce_30_series}.

% Due to the fact that the computations in rendering techniques do not require high accuracy as lower precision only produces negligible differences in colors or position values, the decision was clear to use single precision floating point numbers in the development of the ray tracer for the highest possible performance.

% \subsubsection{TornadoVM intrinsic data types}

% TornadoVM provides a set of data types which map directly to the intrinsics found in the backend languages such as OpenCL and CUDA:

% \begin{itemize}
%     \item Data types in the form of \textit{TypeN}, are structures containing an \textit{N} number of variables of type \textit{Type}, where \textit{Type} may take the form of primitive data types such as \texttt{int, float or double}.

%     Example: a \textit{Float3} data type houses 3 float values.
    
%     \item Data types in the form of \textit{VectorTypeN}, are arrays of variables in the form of \textit{TypeN}.
    
%     Example: a \textit{VectorFloat3} object is an array of \textit{Float3} values.
% \end{itemize}

% \subsubsection{3D Vectors}

% 3D Vectors are used for positions and directions throughout the application, which consist of three float values: x, y and z components.

% To represent a set of float values, TornadoVM's intrinsic \textit{FloatN} data types were considered due to the performance optimizations of built-in data structures \cite{nvidia-pg:2022}.

% While it would be intuitive to use Float3 values to depict 3D vectors and colors containing exactly 3 elements, 3 adjacent float values are stored in $3 \times 4 = 12$ bytes of memory, which violates GPU coalescing restrictions (12 is not a power of 2), which can cause high levels of inefficiency \cite{nvidia-pg:2022}.

% This led to the decision to instead use the Float4 data type to represent 3D vectors and colors, which are $4 \times 4 = 16$ bytes in contrast, thus staying true to the memory coalescing restrictions. Furthermore, while the first three spaces of the Float4 data structure can be used to represent the 3 values of 3D vectors or colors, the last remaining value can be utilized for an additional flag in return statements such as:

% \begin{itemize}
%     \item The \textit{getIntersection()} function returns a \textit{0} or a \textit{-1} as the fourth value as a boolean flag to indicate whether an intersection exists, while the location of the intersection point is returned in the first three values.
%     \item The \textit{getClosestHit()} function returns the index of the closest intersected object as the fourth value, while the location of the intersection point is returned in the first three values.
% \end{itemize}

% \subsubsection{Colors}

% A digital color is represented by a mix of red, green and blue intensity values all in the range of [0, 1].

% The three float values of colors similarly to 3D Vectors, are encompassed within Float4 data structures throughout the rendering process. The final returned values however, are converted into integer representations for the GUI framework to display (the reason for this is outlined in section \ref{section:canvas}).

% \vspace{-0.2cm}\paragraph{Converting color formats}
% The integer representation of color values essentially encode four integers in the range of [0, 255] denoting the alpha, red, green and blue values into one single variable. As we do not have a need for the alpha (transparency) value, this is set to 255 (FF) during conversion. The following method is used to convert between the float and integer color formats:


% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:xxx},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% int toInt(Float4 color) {
%     int r = (int) (color.getX() * 255);
%     int g = (int) (color.getY() * 255);
%     int b = (int) (color.getZ() * 255);
%     return 0xFF000000 | (r << 16) | (g << 8) | b;
% }
% \end{lstlisting}
% \end{figure}

% The result is one integer that contains the red value in the integer at decimal places 6 and 5, green at the  decimal places 4 and 3 and blue at the decimal places 2 and 1.

\subsection{The render method}

\begin{figure}[t!]
    \begin{lstlisting}[caption={Method signature for the main render method to be accelerated with TornadoVM.},label={listing:renderSignature},captionpos=b,
            xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
Renderer::render
    (pixels:              int[],
    dimensions:           int[],
    camera:               float[],
    rayTracingProperties: int[],
    bodyPositions:        VectorFloat4,
    bodySizes:            VectorFloat,
    bodyColors:           VectorFloat4,
    bodyReflectivities:   VectorFloat,
    skybox:               VectorFloat4,
    skyboxDimensions:     int[]) : void;
\end{lstlisting}
\vspace{-1.5em}

\end{figure}

The entire rendering process described in the design section (\ref{section:design}) is implemented within a method named \textit{render} (shown in Listing~\ref{listing:renderSignature}) with the following input arguments:

\vspace{-0.2cm}\paragraph{pixels}
an integer array of size \texttt{width * height} where the computed color values for every pixel are stored upon executing the method.

\vspace{-0.2cm}\paragraph{dimensions}
a two-element integer array that holds the width and height of the viewport.

\vspace{-0.2cm}\paragraph{camera}
a float array of six elements containing the parameters of the camera such as the $x,y,z$ coordinates, yaw and pitch angle of rotation, and field of view.
% \begin{minted}[fontsize=\footnotesize]{java}
% camera[0]: x coordinate of position
% camera[1]: y coordinate of position
% camera[2]: z coordinate of position
% camera[3]: yaw angle of rotation
% camera[4]: pitch angle of rotation
% camera[5]: field of view angle (FOV)
% \end{minted}

\vspace{-0.2cm}\paragraph{rayTracingProperties} an integer array of size 2, which includes the desired soft shadow sampling size and the desired limit of reflection bounces.
% \begin{minted}[fontsize=\footnotesize]{java}
% rayTracingProperties[0]: soft shadow sample size
% rayTracingProperties[1]: reflection bounce limit
% \end{minted}

\vspace{-0.2cm}\paragraph{bodyPositions, bodySizes, bodyColors and bodyReflectivities}
These four arguments encode the information about all of the objects in the scene; each object is defined using its position, size, color, and reflectivity. 

% The entire set of objects are thus represented within the following data structures:

% \\\\
% \begin{centering}
% \begin{tabular}{@{}>{\bfseries}l l}
% bodyPositions & Float4 array (VectorFloat4) of size $N$ \\ 
% bodySizes & float array (VectorFloat) of size $N$\\
% bodyColors & Float4 array (VectorFloat4) of size $N$\\
% bodyReflectivities & float array (VectorFloat) of size $N$
% \end{tabular}
% \end{centering}
% \\\\
% where $N$ is the number of objects in the scene. As an example, the third object at index 2 would be defined by:

% \begin{minted}[fontsize=\footnotesize]{java}
% Float4 position = bodyPositions.get(2)
% float size = bodySizes.get(2)
% Float4 color = bodyColors.get(2)
% float reflectivity = bodyReflectivities.get(2)
% \end{minted}

\vspace{-0.2cm}\paragraph{skybox}
array of four elements that includes the color values of every pixel of the HDRI skybox image. 
This is used to display the panoramic background instead of a plain color. 

% \vspace{-0.2cm}\paragraph{skyboxDimensions}
% The \textit{skyboxDimensions} argument is an integer array of size 2, which includes the width and height of the skybox texture, used to correctly extract color values from the skybox Float4 array (the skybox Float4 array has the size of \texttt{skyboxDimensions[0] * skyboxDimensions[1]}).
% \begin{minted}[fontsize=\footnotesize]{java}
% skyboxDimensions[0]: width of the skybox image
% skyboxDimensions[1]: height of the skybox image
% \end{minted}

These arguments provide the \textit{render} method with all the required information to produce a final color for every pixel.

\subsection{Accelerating the render method using TornadoVM}

As each process of acquiring a final color for each pixel is independent from one another, 
the main loop iterating over the pixels within the \textit{render} method can be marked with the \textit{@Parallel} annotation~\cite{fumero:2018}.
This instructs the TornadoVM compiler to parallelize the for loop and optimize the code depending on the target architecture (in our case a GPU).
Listing~\ref{listing:render} shows a code snippet that represents the main render method expressed in the TornadoVM API using the \textit{@Parallel} annotation. 
Since there are two loops to be parallelized, the TornadoVM compiler will generate an optimized 2D kernel. 

\begin{figure}[t!]
    \begin{lstlisting}[caption={Main render Java method expressed in TornadoVM.},label={listing:render},captionpos=b,
            xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
Renderer::render(int[] pixels,
                 int[] dimensions,
                 ...args...) {
    ...
    int width = dimensions[0];
    int height = dimensions[1];
    ...
    // Parallel marked loop
    for (@Parallel int x = 0; x < width; x++) {
        for (@Parallel int y = 0; y < height; y++) {
        
            // Compute color
            ray = computeViewRay(x, y);
            color = rayTrace(ray, depth);
            
            // Write the color value to output
            pixels[x + y * width] = toInt(color);
        }
    }
}
\end{lstlisting}
\vspace{-1.5em}
\end{figure}

To execute the code, a \textit{TaskSchedule} is defined as shown in Listing~\ref{listing:renderTasks}.
As shown, the arguments \texttt{camera, rayTracingProperties and bodyPositions} are passed to the \texttt{ts.streamIn()} operator to facilitate the user changing viewpoints and rendering parameters as well as the position of each object to allow for physics to move objects around in the scene.
On the other hand, the \texttt{pixels} argument is passed with \texttt{ts.streamOut()} operator in order for the results of the render method to be copied back to the host device and its memory for display.

\begin{figure}[b!]
    \begin{lstlisting}[caption={TaskSchedule composition for accelerating the Java render method with TorandoVM.},label={listing:renderTasks},captionpos=b,
            xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
TaskSchedule ts = new TaskSchedule("s0");
ts.streamIn(camera, rayTracingProperties, bodyPositions);
ts.task("t0", Renderer::render, pixels,
        dimensions, camera, rayTracingProperties,
        bodyPositions, bodySizes,
        bodyColors, bodyReflectivities,
        skybox, skyboxDimensions);
ts.streamOut(pixels);
\end{lstlisting}
\vspace{-1.5em}
\end{figure}

The ray-tracing application has been entirely written in Java and JavaFX framework~\cite{javafx} using \texttt{Canvas} and \texttt{PixelWriter}.
The \textit{JavaFX Canvas} is an image area defined by \textit{width} and \textit{height} that can be used for drawing, while the \textit{JavaFX PixelWriter} is an interface that defines methods which allow for pixel data to be displayed on the canvas.

The JavaFX GUI updates the UI elements at fixed intervals, usually at the refresh rate of the user's monitor screen, which allows for the interface to respond to user input, producing an interactive experience.
A feature called \texttt{AnimationTimer} is provided with the JavaFX suite, which allows the user to define a subroutine inside a handle method that gets called at every update; frequently used to create animations and game loops.
We make use of this feature to invoke TorandoVM and render the canvas with the updated pixels. 

%This loop is used by the ray tracing application to consecutively render images, producing a real-time experience.

% Through the \texttt{PixelWriter}'s \textit{setPixels} method we write the content of the \textit{pixels} array onto a rectangular area on the canvas encapsulated by the top-left corner 
% (first two arguments) and the bottom right corner (third and fourth argument). 
% As we would like to draw on the entire canvas, these values are set to $(0, 0)$ and $(width, height)$ respectively.
% The \textit{format} argument contains the type of color values within the \textit{pixels} array, which unfortunately does not allow the triple-float color representation that the ray tracing application uses. 
% Instead, a conversion step to an integer representation of color is required at the end of the rendering process to make the output compatible with the PixelWriter.


% \subsubsection{Switching between acceleration setups}

% One outstanding strength of TornadoVM, is the ability to switch the execution between available hardware devices as well as backends at runtime.

% The accelerated method may be defined to run with a specified driver backend (e.g. OpenCL, CUDA-PTX or SPIR-V) on a specified device (e.g. Integrated GPU or dedicated GPU).

% Each setup can been polled using the following code snippet:

% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:xxx5},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% ArrayList<TornadoDevice> devices = new ArrayList<>();
% TornadoRuntimeCI runtime = TornadoRuntime.getTornadoRuntime();
% int numTornadoDrivers = runtime.getNumDrivers();
% for (int i = 0; i < numTornadoDrivers; i++) {
%     TornadoDriver driver = runtime.getDriver(i);
%     int numDevices = driver.getDeviceCount();
%     for (int j = 0; j < numDevices; j++) {
%         TornadoDevice device = driver.getDevice(j);
%         devices.add(device);
%     }
% }
% \end{lstlisting}
% \end{figure}

% Depending on which backend and device is wished to be used, the execution of the accelerated task may be mapped to the selected device by:

% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:xxx6},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% ts.mappAllTo(device);
% \end{lstlisting}
% \end{figure}

% Each subsequent call to \texttt{ts.execute()} will then run on the specified setup.

% The data mapping between the host device and the accelerators however, is saved by TornadoVM, which allows for switching between setups at runtime, which encouraged a dropdown-menu to be added to the application facilitating this feature (See Figure \ref{fig:selection}).

% \begin{figure}[H]
% \centering
%   \includegraphics[width=6cm]{images/implementation/selection.png}
%   \caption{Switching between available devices}
%   \label{fig:selection}
% \end{figure}

% \subsection{The GUI Framework}

% To paint the results of the rendering process while allowing for user interaction, it is required to utilize a graphical user interface (GUI) framework. Choosing between available GUI frameworks in Java was based on 3 key factors:

% \vspace{-0.2cm}\paragraph{Speed} The framework has to provide a canvas where pixel colors can be manually set with high efficiency and performance. This is the most important factor as it directly affects the performance of the rendering engine.

% \vspace{-0.2cm}\paragraph{Ease of use} The framework has to allow for easy creation and management of UI elements as well as intuitive functionality to handle action events such as keyboard presses and mouse movements.

% \vspace{-0.2cm}\paragraph{Relevance} The framework should be up to date and actively maintained, with high popularity and a large community.
% \\\\
% Discussions on GUI frameworks revolve around 3 main contenders that are widely used in the Java community: \textit{AWT, Swing and JavaFX}. Out of these options, \textit{JavaFX} \cite{javafx} proved to be by miles the most suitable toolkit for the purposes of the ray tracing application for the following reasons:

% \begin{itemize}
%     \item JavaFX is the newest, most-cutting edge framework out of the four. Developed directly by Oracle, JavaFX is the latest flagship GUI toolkit that was designed to replace older frameworks like AWT and Swing, making them virtually obsolete today.
%     \item JavaFX has an enormous user base, which means the supporting community is vast.  
%     \item The JavaFX Canvas includes a PixelWriter, which takes an input of an array of pixel colors from the user and flushes all of them to a rectangular area on the screen at once. This functionality is crucial to display renders with the highest possible performance.
%     \item JavaFX contains robust event handling models, which can be easily used to facilitate user interaction.
%     \item JavaFX allows for producing rich, CSS-styled UI-components through the use of FXML, which is an XML-based language that provides the structure for building a user interface separate from application logic. Furthermore, drag \& drop visual tool called Scene Builder \cite{scenebuilder} is available to build GUIs for applications with exceptional ease.
% \end{itemize}

% \subsection{The JavaFX Canvas \& PixelWriter}
% \label{section:canvas}

% The \textit{JavaFX Canvas} is an image area defined by a \textit{width} and \textit{height} that can be drawn on, while a \textit{JavaFX PixelWriter} is an interface that defines methods which allow for pixel data to be displayed on the canvas as follows:

% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:xxx7},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% // Construct canvas & get its pixelWriter
% Canvas canvas = new Canvas(width, height);
% pixelWriter = canvas.getGraphicsContext2D().getPixelWriter();

% // Define the format of the color values in pixels array
% PixelFormat format = PixelFormat.getIntArgbInstance();
        
% // Set pixel colors on the canvas
% pixelWriter.setPixels(0, 0, width, height,
%                       format, pixels);
% \end{lstlisting}
% \end{figure}

% The PixelWriter's \textit{setPixels} method writes the content of the \textit{pixels} array onto a rectangular area on the canvas encapsulated by the top-left corner (first two arguments) and the bottom right corner (third and fourth argument). As we would like to draw on the entire canvas, these values are set to $(0, 0)$ and $(width, height)$ respectively.

% The \textit{format} argument contains the type of color values within the \textit{pixels} array, which unfortunately does not allow the triple-float color representation that the ray tracing application uses. Instead, a conversion step to an integer representation of color is required at the end of the rendering process to make the output compatible with the PixelWriter.

% \subsection{The JavaFX loop}

% The JavaFX GUI updates UI elements at fixed intervals, usually at the refresh rate of the user's monitor screen, which allows for the interface to respond to user input, producing an interactive experience.

% An feature called the \textit{AnimationTimer} is provided with the JavaFX suite, which allows the user to define a subroutine inside a \textit{handle} method that gets called at every update, frequently used to create animations and game loops.

% This loop is used by the ray tracing application to consecutively render images, producing a real-time experience:

% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:xxx2},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% new AnimationTimer() {
%     @Override
%     public void handle(long now) {
%         // Render output to pixels array
%         ts.execute();
%         // Set the colors on the canvas
%         pixelWriter.setPixels(0, 0, width, height,
%                               format, pixels, 0, width);
%     }
% }.start();
% \end{lstlisting}
% \end{figure}

% \subsection{Multi-threading}

% One downside of the AnimationTimer however, is that it runs on the same thread that handles UI updates in the background. What this entails is that when there exists a call to a subroutine inside the \textit{handle} method, which takes a longer time to finish, then the UI elements like sliders and menus end up freezing while the routine is executing.

% In our case, this means if rendering a frame takes a whole second, then the entire UI will also be only updating once every second, causing a unresponsive experience.

% To solve this, multi-threading was introduced by spawning a separate render thread where the \texttt{ts.execute()} call is moved, allowing for the UI to continue updating its states while the rendering finishes.

% \subsubsection{Race conditions}

% Having multiple threads however, came with a couple of unwanted side effects. As now the UI thread may run at speeds much faster than the render thread, the UI thread ends up writing new data to the inputs of the render method faster than it can complete a full image.

% The resulting effect is that different portions of the image end up being rendered with different parameters causing artefacts as shown in Figure \ref{fig:race-conditions}.

% \begin{figure}[H]
% \centering
%   \includegraphics[width=\linewidth]{images/implementation/race-condition.png}
%   \caption{Artefacts from race conditions}
%   \label{fig:race-conditions}
% \end{figure}

% This phenomenon is called a \textit{race condition}, whereby two or more threads can access shared data and perform read and write operations at different speeds, leading to synchronization issues.

% To solve this, a form of \textit{double buffering} was implemented.

% \subsubsection{Double buffering}

% To avoid multiple threads reading and writing to the same data locations, double buffering solves the problem by making copy of the shared data to a separate memory space and only allow each thread to read and write to their own assigned data locations.
% When needed, the data is synchronized between the two buffers.


% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:doubleBuffering},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% volatile boolean renderReady = false;
% // Render loop
% new Thread() -> {
%     while (true) {
%         if (!renderReady) {
%             // Copy the data from the second buffer
%             copyDataToBuffer();
%             // Render to pixels array
%             ts.execute();
%             // Signal drawing loop to draw the result
%             renderReady = true;
% }}}.start();
% // Drawing loop
% new AnimationTimer() {
%     @Override
%     public void handle(long now) {
%         if (renderReady) {
%             // Set the colors on the canvas
%             pixelWriter.setPixels(0, 0, width, height,
%                                   format, pixels, 0, width);        
%             // Signal render loop to render next frame
%             renderReady = false;
% }}}.start();
% \end{lstlisting}
% \end{figure}

% With about 10 objects in the scene, the overhead of copying data between the buffers were only recorded to consume about 6.239E-5 ms at each frame, which is a negligible amount that does not noticeably impact performance.

% \subsection{User interaction}

% The final step to the implementation of the application was the addition of user interactivity. There are two main ways the user can change the scene at runtime:

% \begin{itemize}
%     \item Interact with UI elements such as sliders to adjust available parameters
%     \item Use mouse to look-around and keyboard controls to move around the scene in the manner of a first-person camera
% \end{itemize}

% \subsubsection{Sliders}

% Sliders are UI elements that allow users to select values in a specified range (See Figure \ref{fig:sliders}). In JavaFX, users can define a listener that invokes a subroutine whenever a new value is selected. The following example illustrates how a slider is set up to adjust the shadow sample size used throughout the rendering process:

% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:xxx9},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% shadowSampleSizeSlider.valueProperty()
% .addListener((observable, oldValue, newValue) ->
%     shadowSampleSize = newValue.intValue());
% \end{lstlisting}
% \end{figure}


% \begin{figure}[H]
% \centering
%   \includegraphics[width=6.5cm]{images/implementation/Screenshot from 2022-04-28 19-10-26.png}
%   \caption{Settings panel with sliders to adjust settings}
%   \label{fig:sliders}
% \end{figure}

% \subsubsection{First-person camera}

% To allow the user to freely move around the scene, a first-person camera was implemented with the use of JavaFX event handlers. The free camera user control consists of two parts:

% \vspace{-0.2cm}\paragraph{Changing the look direction using the mouse}
% The direction towards which the user is looking is defined by the yaw and pitch rotations of the camera. The behavior of a first-person camera is that the view directions change according to which way the cursor is moved on the screen (e.g moving the mouse from bottom to top will make the camera look upwards).

% This behavior is implemented by recording mouse positions on the event that the mouse is dragged across the canvas:

% \begin{itemize}
%     \item The change in the x coordinate of the mouse position indicates how much the mouse moved horizontally and is thus added to the yaw angle of the camera rotation
%     \item The change in the y coordinate of the mouse position indicates how much the mouse moved vertically and is thus added to the pitch angle of the camera rotation
% \end{itemize}

% \vspace{-0.2cm}\paragraph{Moving camera position using keyboard buttons}
% Moving around the scene is dependent on the direction the user is currently looking towards as the notions of forward, backward, left and right are dependent on which direction the camera is pointing at.

% This entails a computation of a forward vector, which can be derived from the yaw and pitch rotation of the camera:


% Subsequently the vectors pointing left and right can be acquired from the forward vector and the vector defining the up direction, which in our case is simply a unit vector pointing upwards in the y-direction (Note: the cross product of two vectors $a$ and $b$ is a vector that is perpendicular to both):

% \begin{figure}[t!]
%     \begin{lstlisting}[caption={XXX Caption.},label={listing:xxx10},captionpos=b,
%             xleftmargin=.023\textwidth,xrightmargin=.023\textwidth,language=Java]
% fwdVector = normalise(vec3(sin(yaw) * cos(pitch),
%                            sin(pitch),
%                            cos(yaw) * cos(pitch)));
% upVector = vec3(0, 1, 0);

% leftVector = normalise(cross(fwdVector, upVector));
% rightVector = normalise(cross(upVector, fwdVector));

% \end{lstlisting}
% \end{figure}

==> sections/maths.tex <==
\section{Involved mathematics}

In this section, the underlying mathematics required to understand the algorithms within the rendering process of the ray tracer is briefly outlined. This includes the introduction of definitions and equations regarding 3-dimensional geometry, vector operations and ray intersection checks.

Note that throughout this section, figures depicting mathematical processes are 2-dimensional representations, but the basis of the theories carry over to the 3rd dimension as well.

\subsection{3D vectors \& operations}

A \textit{3D vector} is a directed line segment in Euclidean space with a length and a direction, frequently represented by an arrow, connecting an initial point ${A(a_1, a_2, a_3)}$ (also referred to as the \textit{head}) and a terminating point ${B(b_1, b_2, b_3)}$ (also referred to as the \textit{tail}) in a 3-dimensional Cartesian coordinate system.

The 3D vector is a crucial underlying entity in ray tracing that can be used to represent ray directions. Some of the core mathematical concepts required to cover further sections are as follows:

\subsubsection{Vector from two points in space}

Given an initial point \textit{A} and a terminal point \textit{B} in 3D space, the vector $\overrightarrow{AB}$ connecting \textit{A} to point \textit{B} is given by subtracting \textit{A} from \textit{B} \cite{direction_vector}:
\begin{gather*}
\overrightarrow{AB} = B - A
\end{gather*}
This operation is crucial for the constructing of rays in between two points (e.g. given the position of a light source and the position of a point on an object's surface, a directional vector can be computed that travels from the surface point to the light).

\subsubsection{Vector addition and subtraction}
\label{section:vector-add-sub}

Given two vectors \textit{a} and \textit{b},
\begin{itemize}
    \item If the two vectors are positioned in a way where the tail of vector \textit{a} lies on the same point as the head of vector \textit{b}, then the vector pointing from the head of vector \textit{a} to the tail of vector \textit{b} is the resultant vector from the addition of \textit{a} and \textit{b}.
    \item If the two vectors are positioned in a way where the heads of vector \textit{a} and \textit{b} fall onto the same point, then the vector pointing from the tail of vector \textit{a} to the tail of vector \textit{b} is equal to the difference vector \textit{b - a}.
    
    Similarly, the vector pointing from the tail of vector \textit{b} to the tail of vector \textit{b} is equal to the difference vector \textit{a - b}.
\end{itemize}
See Figure \ref{fig:vector-add-sub} for an illustation of the mentioned processes. 
\begin{figure}[H]
\centering
  \includegraphics[width=\linewidth]{images/maths/vector-add-sub.png}
  \caption{Addition and subtraction of two vectors \cite{vector_add_sub}}
  \label{fig:vector-add-sub}
\end{figure}

\subsubsection{Magnitude of a vector}

The length of a vector, in other words the distance between its head and tail points is also referred to as its \textit{magnitude} \cite{vector_magnitude}. The magnitude of a given vector \textit{a} is denoted as $\| a \|$.

The following equation is used to compute the length of a 3D vector $a(a_1, a_2, a_3)$, derived from the \textit{Pythagorean theorem} \cite{vector_magnitude}:
\begin{gather*}
\| a \| = \sqrt{a_1^2 + a_2^2 + a_3^2}
\end{gather*}
The ability to acquire the length of a vector is used by the rendering process to determine the distance in between two points. This is necessary for instance in acquiring the closest intersection point in a ray's path.

\subsubsection{Unit vectors, direction vectors and normalisation}

A \textit{unit vector} is a vector that has a magnitude of exactly 1. Given a given vector \textit{a}, a division with its magnitude yields a unit vector $\hat{u}$, which retains the direction of \textit{a}, but changes it's magnitude to 1. This process is known as \textit{normalisation}:
\begin{gather*}
\hat{u} = \frac{a}{\| a \|}
\end{gather*}
Within the realm of vector operations, to ensure consistency, \textit{direction vectors} would typically be modelled as unit vectors with the initial point situated at the origin \textit{O(0, 0, 0)} of the coordinate system and a terminal point exactly at length 1 away from the origin $O$.

\subsubsection{Dot product of two vectors}
\label{section:dot-product}

Given two vectors \textit{a} and \textit{b}, the \textit{dot product} (also known as the \textit{inner product}) is a single value computed using the two vectors, where the geometric definition is as follows \cite{spiegel:1980}:
\begin{gather*}
a \cdot b = \| a \| \times \| b \| \times cos(\theta)
\end{gather*}
where:
\begin{itemize}
    \item $a \cdot b$ denotes the dot product between \textit{a} and \textit{b}
    \item $\| a \|$ and $\| b \|$ are the magnitudes of \textit{a} and \textit{b} respectively
    \item $\theta$ is the angle in between \textit{a} and \textit{b}
\end{itemize}
Geometrically, the dot product of $a$ and $b$ yields the magnitude of the vector projected from $a$ onto $b$ (See Figure \ref{fig:dot}). 
\begin{figure}[H]
\centering
  \includegraphics[width=5cm]{images/maths/dot.png}
  \caption{The dot product yields the length of a projected vector}
  \label{fig:dot}
\end{figure}
It can be deduced, that in the cases where the dot product of two unit vectors are taken, both $\| a \|$ and $\| b \|$ are equal to 1, which evaluates the equation to:
\begin{gather*}
a \cdot b = cos(\theta)
\end{gather*}
This entails that the dot product of two direction vectors indicates the angular distance in between, where the larger the dot product, the larger the angle. This will prove especially convenient during the computation of shading effects.

\subsubsection{Reflecting a vector off of a surface}
\label{section:vector-refl}

Throughout the implementation of the ray tracer, there are many instances where a reflection ray has to be generated that bounces off of a surface, where two inputs are given:
\begin{itemize}
    \item The direction of the incoming \textit{incident ray}, denoted by \textit{i}
    \item The \textit{normal vector} of the surface, denoted by \textit{n}, this is the unit vector perpendicular to the given surface point
\end{itemize}
The task is then to compute the direction vector \textit{r}, which is reflected off of the surface point symmetrically at the same angle of $\theta$ with respect to the normal vector $n$ as the incoming incident vector \textit{i}.

See Figure \ref{fig:vector-reflection} for the illustration of the process.
\begin{figure}[H]
\centering
  \includegraphics[width=\linewidth]{images/maths/reflection.png}
  \caption{Reflecting a vector around a surface normal}
  \label{fig:vector-reflection}
\end{figure}
Recall the operations of vector addition and subtraction from section \ref{section:vector-add-sub}, according to which vectors \textit{i} and \textit{r} can be expressed with the following formulae:
\begin{gather*}
i = a - b\\
r = a + b
\end{gather*}
Notice that vector \textit{b} can be expressed from vector \textit{i}, normal vector \textit{n} and the cosine of the angle $\theta$ as follows:
\begin{gather*}
b = \| i \| \times cos(\theta) \times n
\end{gather*}
As it is presumed that \textit{i} is a unit vector, its magnitude evaluates to one, which leaves:
\begin{gather*}
b = cos(\theta) \times n
\end{gather*}
The result can then be substituted into the original equations:
\begin{gather*}
i = a - cos(\theta) \times n\\
r = a + cos(\theta) \times n
\end{gather*}
Deriving \textit{a} from the first equation, the reflection vector \textit{r} can be expressed as:
\begin{gather*}
r = i + cos(\theta) \times n + cos(\theta) \times n\\
r = i + 2 \times cos(\theta) \times n
\end{gather*}
Cosine values in trigonometry dictate that:
\begin{gather*}
cos(\theta) = -cos(180 \degree - \theta)
\end{gather*}
Observe that the angle between vector \textit{n} and incident vector \textit{i} is exactly $180 \degree - \theta$, and as both \textit{n} and \textit{i} are presumed to be unit vectors, $cos(180 \degree - \theta)$ can be substituted with the dot product of \textit{n} and \textit{i}:
\begin{gather*}
cos(\theta) = -(\| a \| \times \| b \| \times cos(180 \degree - \theta))\\
cos(\theta) = -(n \cdot i)
\end{gather*}
The final formulae for the reflection vector \textit{r} can thus be written as:
\begin{gather*}
r = i - 2 \times (n \cdot i) \times n
\end{gather*}

\subsubsection{Angular rotation of vectors}
\label{section:rotaions}

A 3D vector can be rotated around any of the three orthogonal axes of a Cartesian coordinate system given an angle in radians (See Figure \ref{fig:rotations}) \cite{rotations}.
\begin{itemize}
    \item The rotation about the $z$-axis is called the $yaw$
    \item The rotation about the $y$-axis is called the $pitch$
    \item The rotation about the $x$-axis is called the $roll$
\end{itemize}

\begin{figure}[H]
\centering
  \includegraphics[width=3.5cm]{images/maths/rotations.jpg}
  \caption{Yaw, pitch and roll rotations \cite{rotations}}
  \label{fig:rotations}
\end{figure}

In our ray tracing application, the direction the camera is looking at is defined with a yaw and pitch value, where angular rotations are necessary to compute the look direction vector.

Given an initial vector $d_1(x_1, y_1, z_1)$ and a $yaw$ angle $\alpha$ as well as a $pitch$ angle $\beta$ in radians, a direction vector $d_2(x_2, y_2, z_2)$ resulting from rotating vector $d_1$ around the $yaw$ and the $pitch$ values can be computed as follows:

\begin{itemize}
    \item The pitch rotation ($y$-direction) is performed by:
    \begin{gather*}
    y_2 = y_1 \times cos(\beta) - z_1 \times sin(\beta)\\
    z_2 = y_1 \times sin(\beta) + z_1 \times cos(\beta)
    \end{gather*}
    \item Then the yaw rotation ($z$-direction) is performed by:
    \begin{gather*}
    x_2 = x_1 \times cos(\alpha) + z_2 \times sin(\alpha)\\
    z_2 = -x_1 \times sin(\alpha) + z_2 \times cos(\alpha)
    \end{gather*}
\end{itemize}

The equations were adapted from the rotation matrices given by the \textit{Yaw, pitch, and roll rotations} article of Steven M. LaValle \cite{rotations}.

\subsection{Rays \& intersection functions}
\label{section:intersection-functions}

A ray in 3D geometry is a path of infinite length in 3D space defined by an \textit{origin} point and a \textit{direction} vector.

On a path of a ray with origin $O$ and direction $d$, any point $P$ may be expressed as the equation:
\begin{gather*}
P = O + d \times t
\end{gather*}
where $t$ is a value which denotes the length from origin point $O$ to point $P$.

Given a defined ray and a primitive shape, an intersection function should return whether the ray intersects with the shape and provide the point of intersection when it exists.

\subsubsection{Ray-Sphere intersection}

A sphere is defined by the location of its center point called the \textit{origin} and its \textit{radius}.

Given a sphere with origin point $C$ and radius $R$, and a ray with origin point $O$ and direction $d$, the geometrical solution of the intersection check is as follows (Refer to Figure \ref{fig:ray-sphere} throughout the solution):
\begin{figure}[H]
\centering
  \includegraphics[width=6.5cm]{images/maths/ray-sphere.png}
  \caption{Ray-sphere intersection check}
  \label{fig:ray-sphere}
\end{figure}
\noindent Recall from section \ref{section:vector-add-sub} that vector $\overrightarrow{OC}$ can be computed as:
\begin{gather*}
\overrightarrow{OC} = O - C
\end{gather*}
As vector $\overrightarrow{OP}$ is a projection of vector $\overrightarrow{OC}$ onto vector $d$, recall from section \ref{section:dot-product} that $\overrightarrow{OP}$ can be expressed as the dot product of $\overrightarrow{OC}$ and $d$:
\begin{gather*}
\overrightarrow{OP} = (O - C) \cdot d
\end{gather*}
Point $P$ can then be expressed as:
\begin{gather*}
P = O + d \times \| \overrightarrow{OP} \|\\
P = O + d \times \| (O - C) \cdot d \|
\end{gather*}
With the location of point $P$ computed, vector $\overrightarrow{CP}$ can be obtained. Here the first line of the intersection check can be performed:
\begin{itemize}
    \item In the case that $\| \overrightarrow{CP} \|$ is larger than the radius $R$ of the sphere, point $P$ lies outside the sphere and no intersection occurs.
    \item Otherwise, an intersection occurs, and the new task becomes the computation of intersection point $Q$.
\end{itemize}
Notice how points $C$, $P$ and $Q$ form a right-angled triangle (a triangle that contains a 90\degree~angle), where the hypotenuse $\| \overrightarrow{CQ} \|$ is equal to the radius $R$ of the circle and the opposite $\| \overrightarrow{CP} \|$ has already been computed. This allows for the use of the Pythagorean theorem for the calculation of length $\| \overrightarrow{PQ} \|$:
\begin{gather*}
\| \overrightarrow{PQ} \| = \sqrt{R^2 - \| \overrightarrow{CP} \| ^2}
\end{gather*}
The magnitude $\| \overrightarrow{OQ} \|$ can then be obtained from a simple subtraction:
\begin{gather*}
\| \overrightarrow{OQ} \| = \| \overrightarrow{OP} \| - \| \overrightarrow{PQ} \|
\end{gather*}
\begin{itemize}
    \item In the case where $\| \overrightarrow{OQ} \|$ is negative, the origin point $O$ has to be located inside the sphere, meaning that the the ray starts from within the object itself. For the purposes of this application, these instances are not classified as as intersection.
    \item Otherwise, the location of point $Q$ can then be directly evaluated from:
            \begin{gather*}
            Q = O + d \times \| \overrightarrow{OQ} \|
            \end{gather*}
\end{itemize}


\subsubsection{Ray-Plane intersection}
\label{section:ray-plane-isect}

The ray tracing application is built to support a plane in the scene that is parallel to the $xz$ plane (the $xz$ plane is the plane where every point has a $y$ value of 0), in other words is perfectly horizontal. Such a plane is defined by a single $height$ value, denoting the $y$ coordinate of every point on the plane.

Given a plane with height $h$, and a ray with origin point $O$ and direction $d$, the solution of the intersection check is as follows:
(Refer to Figure \ref{fig:ray-plane} throughout the solution):
\begin{figure}[H]
\centering
  \includegraphics[width=6.5cm]{images/maths/ray-plane.png}
  \caption{Ray-plane intersection check}
  \label{fig:ray-plane}
\end{figure}
Notice how due to triangle similarity, a ratio $t$ can be expressed as:
\begin{gather*}
t = \frac{\| \overrightarrow{OQ} \|}{\| d \|} = \frac{O_y - P_y}{d_y}
\end{gather*}
where $d_y$ is the $y$ component of direction vector $d$, and $O_y$ and $P_y$ are the $y$ components of points $O$ and $P$ respectively.

As direction vector $d$ is a unit vector, $\| d \|$ evaluates to 1, and as it is known that every point on the plane has a $y$ component equal to height $h$, the statement can be simplified to:
\begin{gather*}
t = \| \overrightarrow{OQ} \| = \frac{O_y - h}{d_y}
\end{gather*}
Here, the following occurrences can be observed:
\begin{itemize}
    \item In the case where the ratio $t$ is less than $0$, direction $d$ points away from the plane and no intersection is found.
    \item Otherwise, an intersection occurs, and the new task becomes the computation of intersection point $Q$.
\end{itemize}
Intersection point $Q$ can simply be derived from the definition of a point on a ray's path as:
\begin{gather*}
Q = O + d \times \| \overrightarrow{OQ} \|\\
Q = O + d \times \frac{O_y - h}{d_y}
\end{gather*}

\subsection{The normal vector of a surface - 400}
As stated in section \ref{section:vector-refl}, a normal vector of a surface is a unit vector perpendicular to a given point on the surface. For different primitives, given a surface point $P$, the normal vector $n$ at point $P$ are computed as follows:

\subsubsection{Normal of a sphere - 100}

Given a sphere with origin point $C$ and a point $P$ on its surface, regardless of the radius of the sphere, it is trivial that the normal of surface point $P$ points in the same direction as vector $\overrightarrow{CP}$ (See Figure \ref{fig:sphere-normal}).
\begin{figure}[H]
\centering
  \includegraphics[width=5cm]{images/maths/sphere-normal.png}
  \caption{Normal vector at a given point on a sphere}
  \label{fig:sphere-normal}
\end{figure}
The normal vector $n$ can thus be expressed as the normalised version of vector $\overrightarrow{CP}$:
\begin{gather*}
n = \frac{\overrightarrow{CP}}{\| \overrightarrow{CP} \|}
\end{gather*}

\subsubsection{Normal of a plane - 100}

As stated before in section \ref{section:ray-plane-isect}, the supported plane in the application is parallel to the $xz$ plane, which entails that the normal vector of our plane at any given point on its surface is simply one that points directly upwards in the Y direction:
\begin{gather*}
n = (0, 1, 0)
\end{gather*}
